What do Neural Machine Translation Models Learn about Morphology?

Neural machine translation (MT) models obtain state-of-the-art performance while maintaining a simple, end-to-end architecture. However, little is known about what these models learn about source and target languages during the training process. In this work, we analyze the representations learned by neural MT models at various levels of granularity and empirically evaluate the quality of the representations for learning morphology through extrinsic part-of-speech and morphological tagging tasks. We conduct a thorough investigation along several parameters: word-based vs. character-based representations, depth of the encoding layer, the identity of the target language, and encoder vs. decoder representations. Our data-driven, quantitative evaluation sheds light on important aspects in the neural MT system and its ability to capture word structure.

==> motivation.tex <==
\section{Motivation} \label{sec:motivation}

Translating morphologically-rich languages is especially difficult due to a large vocabulary size and a high level of sparsity.  Different solutions have been proposed to deal with this problem, for example factored models in phrase-based MT~\cite{koehn-hoang:2007:EMNLP-CoNLL2007} or softmax approximations in neural MT~\cite{ruder-softmax}. More recently, neural MT systems have shown significant gains by exploiting characters and other sub-word units~\cite{costajussa-fonollosa:2016:P16-2,sennrich-haddow-birch:2016:P16-12,wu2016google}. Presumably, such models are better than word-based models in representing the structure of rare and unseen words. Indeed, \newcite{sennrich-haddow-birch:2016:P16-12} have found that the unigram translation accuracy of words decreases for lower-frequency words. They also observed somewhat different behavior when translating into different languages. It is less clear, however, what and how neural translation models learn about word structure. In this work we are interested in answering questions such as the following:
\begin{itemize}
\item How do character-based models improve neural MT?
\item What components of the NMT system encoder word structure? 
\item How does the target language affect the learning of word structure?
\item What is the role of the decoder in learning word representations?
\end{itemize}

In the next section, we describe our data-driven approach for addressing such questions. We aim to obtain quantitative answers that will lead to generalizable conclusions. 


